Efficient Dialogue State Tracking by Selectively Overwriting Memory

Recent works in dialogue state tracking (DST) focus on an open vocabulary-based setting to resolve scalability and generalization issues of the predefined ontology-based approaches. However, they are inefficient in that they predict the dialogue state at every turn from scratch. Here, we consider dialogue state as an explicit fixed-sized memory and propose a selectively overwriting mechanism for more efficient DST. This mechanism consists of two steps: (1) predicting state operation on each of the memory slots, and (2) overwriting the memory with new values, of which only a few are generated according to the predicted state operations. Our method decomposes DST into two sub-tasks and guides the decoder to focus only on one of the tasks, thus reducing the burden of the decoder. This enhances the effectiveness of training and DST performance. Our SOM-DST (Selectively Overwriting Memory for Dialogue State Tracking) model achieves state-of-the-art joint goal accuracy with 51.72% in MultiWOZ 2.0 and 53.01% in MultiWOZ 2.1 in an open vocabulary-based DST setting. In addition, we analyze the accuracy gaps between the current and the ground truth-given situations and suggest that it is a promising direction to improve state operation prediction to boost the DST performance.

==> figs/overview_macroscopic.tex <==
\begin{figure}[t] 
\centering
\includegraphics[width=0.5\textwidth]{overview3}
\caption{The overview of the proposed \ours{}. \ours{} takes the dialogue of the previous and current turn, and the previous dialogue state, and outputs the current dialogue state. This is performed by two sub-components: \sop{} and \svg{}. Only the slots on which \operation{update} operation needs to be performed become the input to the slot value generator, thus making our framework efficient.}
\label{fig:overview}
\end{figure}

==> figs/overview_microscopic.tex <==
\begin{figure}[t] 
\centering
\includegraphics[width=0.5\textwidth]{model}
\caption{The overview of our \ours{}. \ours{} consists of two components: (1) \sop{} and (2) \svg{}. \SOP{} takes the dialogue of the previous and current turn with the previous turn dialogue state and predicts the operations to perform on each of the slots. Domain classification is jointly performed as an auxiliary task. \SVG{} generates the values for the slots that take \operation{update} as the predicted operation. Value generation for a slot is done in an autoregressive manner.}
\label{fig:model}
\end{figure}

==> tabs/ablation_two_columns.tex <==
\begin{table}[!t]
    \centering
    \label{table:ablation-study}
    \caption{
        Joint goal accuracy on the MultiWOZ 2.1 test set when the four-way state operation prediction changes to two-way or six-way.
        % (-) means changing a component of \ours{}, and (+) means using the ground truth instead of the prediction to measure the upper bound of the performance.
    }
    \label{table:ablation}
    \footnotesize
    \begin{threeparttable}
    \begin{tabular*}{\columnwidth}{l@{\extracolsep{\fill}}r}
        \toprule
        Choice of State Operations & Joint Accuracy \\
        \midrule
        Four - \operation{carryover}, \operation{delete}, \operation{dontcare}, \operation{update} & 53.01 \\
        \midrule
        % \quad (-) Exclude domain classification   & 49.38 \\
        Two - \operation{carryover}, \operation{non-carryover} & 52.06 \\
        Six - \operation{carryover}, \operation{delete}, \operation{dontcare}, \operation{update}, \operation{yes}, \operation{no} & 52.97 \\
        % \midrule
        % \quad Use BERT-Large    & 53.98 \\
        \bottomrule
    \end{tabular*}
    \end{threeparttable}
\end{table}
